Reliable and Responsible Foundation Models: A Comprehensive Survey

Foundation models, including Large Language Models (LLMs), Multimodal Large Language Models (MLLMs), Image Generative Models (i.e, Text-to-Image Models and Image-Editing Models), and Video Generative Models, have become essential tools with broad applications across various domains such as law, medicine, education, finance, science, and beyond. As these models see increasing real-world deployment, ensuring their reliability and responsibility has become critical for academia, industry, and government. This survey addresses the reliable and responsible development of foundation models. We explore critical issues, including bias and fairness, security and privacy, uncertainty, explainability, and distribution shift. Our research also covers model limitations, such as hallucinations, as well as methods like alignment and Artificial Intelligence-Generated Content (AIGC) detection. For each area, we review the current state of the field and outline concrete future research directions. Additionally, we discuss the intersections between these areas, highlighting their connections and shared challenges. We hope our survey fosters the development of foundation models that are not only powerful but also ethical, trustworthy, reliable, and socially responsible.

==> tables/reference.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=white, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

    
\begin{figure}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
        forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                text centered,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center}
            },
            where level=1{text width=15em,font=\normalsize}{},
            where level=2{text width=14em,font=\normalsize}{},
            where level=3{text width=15em,font=\normalsize}{},
            where level=4{text width=15em,font=\normalsize}{},
            where level=5{text width=15em,font=\normalsize}{},
            [
                Latent Reasoning, ver
                [
                    Preliminary: Latent \\Chain-of-Thought (\S\ref{sec:preliminary})
                    [
                        General Framework
                    ]
                    [
                        Connections to Explicit \\Chain-of-Thought
                    ]
                    [
                        Latent Reasoning Updates \\of Diffusion Models
                    ]
                ]
                [
                    Latent Reasoning (\S\ref{sec:latent cot reasoning})
                    [
                        Activation-based \\Recurrent Methods
                        [
                            Architectural Recurrence
                            [
                                Universal Transformer~\citep{dehghani2018universal}{, }
                                CoTFormer~\citep{mohtashami2023cotformer}{, }\\
                                Recursive Transformer~\citep{bae2024relaxed}{, }
                                AlgoFormer~\citep{gao2024algoformer}{, }
                                Recurrent-Depth~\citep{geiping2025scaling}
                                , leaf,text width=40em
                            ]
                        ]
                        [
                            Training-induced Recurrence
                            [
                                Coconut~\citep{hao2024training}{, }
                                CODI~\citep{shen2025codi}{, }VO-VAE~\citep{su2025token}{, }
                                CCOT~\citep{cheng2024compressed}{, }Decomposes Reasoning ~\citep{jin2024disentangling}{, }
                                \\Light thinker\citep{zhang2025lightthinker}{, }
                                Filler Tokens~\citep{pfau2024lets}{, }
                                Pause Tokens~\citep{goyal2024think}{, }
                                Planning Token~\citep{wang2024guiding}
                                , leaf,text width=40em
                            ]    
                        ]
                        [
                            Training Strategies \\for Recurrent Reasoning
                            [
                                MIDAS~\citep{saunshi2024inductive}{, }
                                Looping-Inspired Regularization~\citep{saunshi2025reasoning}{, }\\
                                Stepwise Internalization~\citep{deng2024explicit}{, }
                                Coconut~\citep{hao2024training}{, }
                                RELAY~\citep{yu2025enhancing}
                                , leaf,text width=40em
                            ]
                        ]
                        [
                            Applications and Capabilities
                            [
                                Looped Architectures~\citep{schwarzschild2021can,giannou2023looped} {, }
                                Looped Transformers~\citep{de2024simulation}{, }
                                Planning Tokens~\citep{wang2024guiding}{, }\\
                                Decomposes Reasoning~\citep{jin2024disentangling}{, }
                                Optimization and Meta-Learning~\citep{gatmiry2024can, chen2024bypassing}
                                , leaf,text width=40em
                            ]
                        ]
                    ]
                    [
                        Temporal Hidden-\\state Methods
                        [
                            Linear-State Recurrence
                            [
                                Linear Attention~\citep{katharopoulos2020transformers}{, }
                                RetNet~\citep{sun2023retentive}{, }
                                GLA~\citep{yang2023gated}{, }
                                RWKV-6~\citep{peng2024eagle}{, }\\
                                HGRN-2~\citep{qin2024hgrn2}{, }
                                Mamba-2~\citep{dao2024transformers}{, }
                                DeltaNet~\citep{yang2024deltanet}{, }
                                Gated DeltaNet~\citep{yang2024gateddeltanet}
                                , leaf,text width=40em
                            ]
                        ]
                        [
                            Gradient-State Recurrence
                            [
                                TTT~\citep{sun2024ttt}{, }Titans~\citep{behrouz2024titans}{, }ATLAS~\citep{behrouz2025atlas}{, }Gated delta~\citep{yang2024gateddeltanet}{, }Soft Reasoning~\cite{zhu2025soft}
                                , leaf,text width=40em
                            ]
                        ]
                        [
                            Training-induced \\Hidden-State Conversion
                            [
                                SUPRA~\citep{mercat2024supra}{, }MOHAWK~\citep{bick2024mohawk}{, }Llamba~\citep{bick2025llamba}{, }LoLCATs~\citep{zhang2024lolcats}{, }Liger~\citep{lan2025liger}
                                , leaf,text width=40em
                            ]
                        ]
                    ]
                ]
                [
                    Mechanical Interpretability (\S\ref{sec:interpretability})
                    [
                        Do Layer Stacks \\Reflect Latent CoT?
                        [
                            Layer Depth Influence \\Reasoning Capabilities
                            [
                            Implicit Reasoning~\citep{yu2024llms}{, } 
                            Two-Hop Reasoning~\citep{guo2025llms}
                            , leaf,text width=40em
                            ]
                        ]
                        [
                            Layer Depth Serves As \\The Primary Bottleneck
                            [
                            Looped Transformers~\citep{saunshi2025reasoning}{,} Log-Depth Transformers~\citep{merrill2025little}
                            , leaf,text width=40em
                            ]
                        ]
                        [
                            Clear Correspondence Between \\Layer Depth and Resoning
                            [
                             MechanisticProbe~\citep{hou2023towards}{, }Back Attention~\citep{yu2025back}{,} \\Iteration Head~\citep{cabannes2024iteration}{,} 
                            Matching Operation~\citep{wang2024towards}
                            , leaf,text width=40em
                            ]
                        ]
                    ]
                    [
                        Mechanisms of Latent CoT \\in Layer Representation
                        [
                            Shallow Layers
                            [
                            Micse~\citep{klein2022micse}{,} Feed-forward Layers~\citep{geva2020transformer}{,} Unveiling Induction Heads~\citep{chen2024unveiling}{,}  Hopping~\citep{biran2024hopping}{,} \\
                            Loss Landscape Geometry~\citep{wang2024loss}{,} Memory Bottleneck~\citep{li2019enhancing}{,} Unpacking Robustness~\citep{walkowiak2025unpacking}{,} \\
                            Multi-hop Reasoning~\citep{yang2024large}{,} Layer by Layer~\citep{skean2025layer}{,} 
                            Distributional Reasoning~\citep{shalev2024distributional}
                            , leaf,text width=40em
                            ]
                        ]
                        [
                            Intermediate Layers
                            [
                            Representation~\citep{skean2024does}{,} Group Operations~\citep{wu2024unifying}{,} Interpretability~\citep{wang2022interpretability}{,} Emergent Abilities~\citep{berti2025emergent}\\Compositional Generalization~\citep{berti2025emergent}{,} 
                            Factual Recall Behaviors~\citep{wang2024unveiling}{,} Test-time Compute~\citep{geiping2025scaling}
                            , leaf,text width=40em
                            ]
                        ]
                        [
                            Deep Layers
                            [
                            Interwoven Structured Knowledge~\citep{lei2025representation}{,} Layer by Layer~\citep{skean2025layer}{,} Gpt-2 ~\citep{hanna2023does}{,} Inheritune~\citep{sanyal2024inheritune}{,} \\Step-by-step~\citep{dutta2024think}{,} Lift~\citep{yuan2024lift}{,} LLM Depth~\citep{csordas2025language}{,} Void in LLM~\citep{shemiranifar2025void}{,} Curse of Depth ~\citep{sun2025curse}
                            , leaf,text width=40em
                            ]
                        ]
                        [
                            Theory of Information Flow
                            [
                            Causal Mediation Analysis~\citep{stolfo2023mechanistic}{,} Edge of Generalization~\citep{wang2024grokked}{,} Back Attention~\citep{yu2025back}
                            , leaf,text width=40em
                            ]
                        ]
                    ]
                    [
                        Limits of Layer-Based \\Latent CoT Interpretation
                        [
                            Proof of Turing completeness\\ in model architectures
                            [
                            RNN encoder-decoder~\citep{Cho2014LearningPhrase}{,} 
                            Transformers~\citep{vaswani2017attention}{,} 
                            Turing Completeness~\citep{perez2019turing}~\citep{qiu2024ask}
                            , leaf,text width=40em
                            ]
                        ]
                    ]
                ]
                [
                    Towards Infinite-depth\\ Reasoning (\S\ref{sec:infinite-depth reasoning})
                    [
                        Spatial Infinite Reasoning:\\ Text Diffusion Models
                        [
                            Masked Diffusion Models
                            [
                                D3PM~\citep{austin2021structured}{,} SEDD~\citep{lou2024discrete}{,} RADD~\citep{ou2024your}{,} MD4~\citep{shi2024simplified}{,} Simple-MDM~\citep{sahoo2024simple}{,} MDM~\citep{nie2024scaling}{,} \\
                                MMaDA~\citep{yang2025mmada}{,} IRED~\citep{Du_2024_ICML}{,} LLaDA~\citep{nie2025large}{,} dKV-Cache~\citep{ma2025dkv}{,} DoT-SEDD~\citep{ye2024diffusionthoughtschainofthoughtreasoning}{,} \\
                                dLLM-Cache~\citep{liu2025dllmcacheacceleratingdiffusionlarge}{,} d1-LLaDA~\citep{zhao2025d1scalingreasoningdiffusion}{,} MGDM~\citep{ye2025autoregressiondiscretediffusioncomplex}{,} LLaDA~1.5~\citep{zhu2025llada15variancereducedpreference}{,} DCoLT~\citep{huang2025reinforcingdiffusionchainlateral}
                                , leaf,text width=40em
                            ]
                        ]
                        [
                            Embedding-based Diffusion \\Models
                            [
                                Diffusion-LM~\citep{li2022diffusionlmimprovescontrollabletext}{,} CDCD~\citep{dieleman2022continuousdiffusioncategoricaldata}{,} Bit Diffusion~\citep{chen2023analogbitsgeneratingdiscrete}{,} Plaid~\citep{gulrajani2023likelihoodbaseddiffusionlanguagemodels}{,} BFN~\citep{graves2025bayesianflownetworks}{,} DoT-Plaid~\citep{ye2024diffusionthoughtschainofthoughtreasoning}{,} \\
                                TESS~\citep{mahabadi2024tesstexttotextselfconditionedsimplex}{,} TESS 2~\citep{tae2025tess}
                                , leaf,text width=40em
                            ]
                        ]
                        [
                            Hybrid AR-Diffusion Models
                            [
                                DiffuLLaMA~\citep{gong2025scaling}{,} Dream~\citep{dream2025}{,} L2D~\citep{cetin2025large}{,} Gemini Diffusion~\citep{google2025geminiDiffusion}{,} Mercury~\citep{labs2025mercuryultrafastlanguagemodels}
                                , leaf,text width=40em
                            ]
                        ]
                    ]
                    [
                        'Infinitely Long' \\Optimizer Network
                        [
                            Infini-attention
                            [
                            Transformers with infini-attention~\citep{munkhdalai2024leave}
                            , leaf,text width=40em
                            ]
                        ]
                        [
                            Test-time training (TTT)\\ and its descendants
                            [
                            TTT~\citep{sun2024ttt}{, }Titans~\citep{behrouz2024titans}{, }OmegaNet and Atlas~\citep{behrouz2025atlas}
                            , leaf,text width=40em
                            ]
                        ]
                        [
                            Implicit Fixed-Point RNNs
                            [
                            Implicit language models are rnns~\citep{schone2025implicit}
                            , leaf,text width=40em
                            ]
                        ]
                    ]
                ]
            ]
        \end{forest}
}
    \caption{Taxonomy of Latent Reasoning.}
    \label{fig:taxo_of_lr}
\end{figure}

==> tables/tree_template_empty.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=white, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
        forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=center,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                text centered,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center}
            },
            where level=1{text width=15em,font=\normalsize}{},
            where level=2{text width=14em,font=\normalsize}{},
            where level=3{text width=15em,font=\normalsize}{},
            where level=4{text width=15em,font=\normalsize}{},
            where level=5{text width=15em,font=\normalsize}{},
            % ================= ROOT =================
            [
                Level 0: Overview, ver
                % ------------- BRANCH 1 -------------
                [
                    Level 1A: Category
                    [
                        Level 2A.1: Subcategory
                        [
                            Level 3A.1.a: Topic
                            [
                                Level 4A.1.a.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3A.1.b: Topic
                            [
                                Level 4A.1.b.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3A.1.c: Topic
                            [
                                Level 4A.1.c.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                    ]
                ]
                % ------------- BRANCH 2 -------------
                [
                    Level 1B: Category
                    [
                        Level 2B.1: Subcategory
                        [
                            Level 3B.1.a: Topic
                            [
                                Level 4B.1.a.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3B.1.b: Topic
                            [
                                Level 4B.1.b.i: Leaf Items, leaf, text width=40em
                            ]    
                        ]
                        [
                            Level 3B.1.c: Topic
                            [
                                Level 4B.1.c.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3B.1.d: Topic
                            [
                                Level 4B.1.d.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                    ]
                    [
                        Level 2B.2: Subcategory
                        [
                            Level 3B.2.a: Topic
                            [
                                Level 4B.2.a.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3B.2.b: Topic
                            [
                                Level 4B.2.b.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3B.2.c: Topic
                            [
                                Level 4B.2.c.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                    ]
                ]
                % ------------- BRANCH 3 -------------
                [
                    Level 1C: Category
                    [
                        Level 2C.1: Subcategory
                        [
                            Level 3C.1.a: Topic
                            [
                                Level 4C.1.a.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3C.1.b: Topic
                            [
                                Level 4C.1.b.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3C.1.c: Topic
                            [
                                Level 4C.1.c.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                    ]
                    [
                        Level 2C.2: Subcategory
                        [
                            Level 3C.2.a: Topic
                            [
                                Level 4C.2.a.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3C.2.b: Topic
                            [
                                Level 4C.2.b.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3C.2.c: Topic
                            [
                                Level 4C.2.c.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3C.2.d: Topic
                            [
                                Level 4C.2.d.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                    ]
                    [
                        Level 2C.3: Subcategory
                        [
                            Level 3C.3.a: Topic
                            [
                                Level 4C.3.a.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                    ]
                ]
                % ------------- BRANCH 4 -------------
                [
                    Level 1D: Category
                    [
                        Level 2D.1: Subcategory
                        [
                            Level 3D.1.a: Topic
                            [
                                Level 4D.1.a.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3D.1.b: Topic
                            [
                                Level 4D.1.b.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3D.1.c: Topic
                            [
                                Level 4D.1.c.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                    ]
                    [
                        Level 2D.2: Subcategory
                        [
                            Level 3D.2.a: Topic
                            [
                                Level 4D.2.a.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3D.2.b: Topic
                            [
                                Level 4D.2.b.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                        [
                            Level 3D.2.c: Topic
                            [
                                Level 4D.2.c.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                    ]
                    [
                        Level 2D.3: Subcategory
                        [
                            Level 3D.3.a: Topic
                            [
                                Level 4D.3.a.i: Leaf Items, leaf, text width=40em
                            ]
                        ]
                    ]
                ]
            ]
        \end{forest}
}
    \caption{Taxonomy (structure-only placeholders). Replace placeholders (e.g., \emph{Level 2B.1: Subcategory}) with your content.}
    \label{fig:taxo_structure_only}
\end{figure}

